StyleGAN-Human: A Data-Centric Odyssey of Human Generation

Unconditional human image generation is an important task in vision and graphics, which enables various applications in the creative industry. Existing studies in this field mainly focus on "network engineering" such as designing new components and objective functions. This work takes a data-centric perspective and investigates multiple critical aspects in "data engineering", which we believe would complement the current practice. To facilitate a comprehensive study, we collect and annotate a large-scale human image dataset with over 230K samples capturing diverse poses and textures. Equipped with this large dataset, we rigorously investigate three essential factors in data engineering for StyleGAN-based human generation, namely data size, data distribution, and data alignment. Extensive experiments reveal several valuable observations w.r.t. these aspects: 1) Large-scale data, more than 40K images, are needed to train a high-fidelity unconditional human generation model with vanilla StyleGAN. 2) A balanced training set helps improve the generation quality with rare face poses compared to the long-tailed counterpart, whereas simply balancing the clothing texture distribution does not effectively bring an improvement. 3) Human GAN models with body centers for alignment outperform models trained using face centers or pelvis points as alignment anchors. In addition, a model zoo and human editing applications are demonstrated to facilitate future research in the community.

==> section/limitations.tex <==
\section{Limitations}
Compared to face generation, training an unconditional human GAN is an arduous task because the semantic features of the full-body are much more complicated than a single face. Figure~\ref{fig:failure_cases} shows some failure cases generated by the baseline model, suggesting several directions that can be strengthened in future human generation work. Artifacts caused by entangled features of faces/hands and clothing accessories are revealed in Figures~\ref{fig:failure_cases} (a) - (c). Case (d) exhibits three hands on a person, which indicates that the global perception of the model needs to be improved~\cite{huang2017beyond}. We observed inferior hand quality in rare poses such as (e) and (f). To address this, the potential work could be augmenting training with such extreme poses, changing the data distribution, or implementing independent networks (i.e. fine-grained discriminators) to enhance local details~\cite{detailmemore}. The face and texture quality in cases (b) and (g) could be enhanced by local refinement as well.
\begin{figure}[t]
  \centering
  \includegraphics[width=\linewidth]{pdf/failure_cases_oneline.pdf}
  \caption{\textbf{Failure cases from baseline model.} (a) - (c): Features such as face, texture and accessories are entangled. (d) Three hands detected on a single person. (e) - (f): Inferior generated hand quality. (g): Face quality could be better.}
  \label{fig:failure_cases}
\end{figure}

